DiffInfinite: Large Mask-Image Synthesis via Parallel Random Patch Diffusion in Histopathology

We present DiffInfinite, a hierarchical diffusion model that generates arbitrarily large histological images while preserving long-range correlation structural information. Our approach first generates synthetic segmentation masks, subsequently used as conditions for the high-fidelity generative diffusion process. The proposed sampling method can be scaled up to any desired image size while only requiring small patches for fast training. Moreover, it can be parallelized more efficiently than previous large-content generation methods while avoiding tiling artifacts. The training leverages classifier-free guidance to augment a small, sparsely annotated dataset with unlabelled data. Our method alleviates unique challenges in histopathological imaging practice: large-scale information, costly manual annotation, and protective data handling. The biological plausibility of DiffInfinite data is evaluated in a survey by ten experienced pathologists as well as a downstream classification and segmentation task. Samples from the model score strongly on anti-copying metrics which is relevant for the protection of patient data.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerNo{The model is only defined in section \ref{sec:method}}
\end{enumerate}


\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code to generate synthetic images will be made available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In the appendix}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In the appendix}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{}
\end{enumerate}

\end{enumerate}

==> dev_links.tex <==
% Gannt chart: https://jsfiddle.net/2ewc7yf8/10/

% Figma: https://www.figma.com/file/gPGw1qxyoi5rMaRGgCMaAg/SyReal?t=awl9nY34XTgHrUGO-0

==> goals/metrics.tex <==
% \subsection{Metrics to evaluate generated images}
% \begin{itemize}
%     \item FID
%     \item IS
%     \item $\alpha$-Precision (fidelity)
%     \item $\beta$-Recall (diversity)
%     \item Authenticity (generalization)
%     \item Wasserstein distance?
% \end{itemize}

==> goals/summary.tex <==
% \section{Goals}
% Define:
% \begin{itemize}
%     \item Visual realism (colour, blur etc), diversity, recall with an external model (AIgnostic) --> computational scores
%     \item Clinical sensibility (clinical meanings) --> (Mihaela)
%     \item Describe pragmatic meaning synthetic data for histopathology
% \end{itemize}

% Ideas:
% \begin{itemize}
%     \item Generate synthetic raw images with different sensor properties
%     \item Generate Slide masks for sub-types macro-structures
%     \item Condition Generative models on masks
% \end{itemize}

==> goals/summary2.tex <==
% \section{Experiments}

% \subsection{Generate histopathology slides}
% \subsection{Generate histopathology slides conditioned on subtypes}
% \subsection{Train on raw data}
% \subsection{Map from one sensor to another}
% \subsection{Generate masks and use is for inpainting}
% \begin{itemize}
%     \item Downsample masks
%     \item train on downsampled masks
%     \item upsample masks
%     \item concatenate generated mask with generated images
% \end{itemize}
% \subsection{From mask to RGB}

==> literature_review.tex <==

% Let's try to use this document to add the most important papers and a short description here already
\section{Related work and work we build on}
How faithful is your Synthetic Data? \cite{alaa2022faithful} \\
Introduces 3-dimensional metric (on sample-level) to evaluate 
\begin{itemize}
    \item $\alpha$-Precision (fidelity)
    \item $\beta$-Recall (diversity)
    \item Authenticity (generalization)
\end{itemize}

Can additionally be used to filter generated samples based on quality (model auditing) \\
Ahmed’s links:
\url{https://www.reddit.com/r/technology/comments/10r31ca/paper} (stable dif f usion memorizes some images/)
%\url{https://windowsontheory.org/2023/02/21/provable−copyright−protection−f or−generative−
%models/}




==> metrics.tex <==
The following metrics are used in \Cref{sec:dass} to assess the fidelity and memorization degree of the model.

\begin{metric}[Improved Precision]
\label{met:ip}
The following metrics are used in \Cref{sec:dass} to assess the fidelity and memorization degree of the model.MetricMetric
Samples from $X_r \sim P_r$ and $X_g \sim P_g$ are drawn and embedded into a high-dimensional feature space per \cite{NEURIPS2019_0234c510}, forming sets of feature vectors $\boldsymbol{\Phi}_r$ and $\boldsymbol{\Phi}_g$. A manifold in the feature space is estimated for each $\boldsymbol{\Phi}$ using pairwise Euclidean distances between feature vectors, and hyperspheres determined by the $k$th nearest neighbor.
\begin{comment}
Following \cite{NEURIPS2019_0234c510}, real and generated samples from $X_r \sim P_r$ and $X_g \sim P_g$ are drawn, respectively, and embedded in a high-dimensional feature space using a pre-trained classifier network. These samples' feature vectors, $\boldsymbol{\phi}_r$ and $\boldsymbol{\phi}_g$, form sets denoted by $\boldsymbol{\Phi}_r$ and $\boldsymbol{\Phi}_g$.

For $\boldsymbol{\Phi} \in \{\boldsymbol{\Phi}_r, \boldsymbol{\Phi}_g\}$, a manifold in the feature space is estimated. This estimation is formed by calculating pairwise Euclidean distances between feature vectors in the set and defining hyperspheres around each feature vector, using the distance to its $k$th nearest neighbor as the radius.

A binary function $f(\boldsymbol{\phi}, \boldsymbol{\Phi})$ is defined to identify whether a given sample $\boldsymbol{\phi}$ is within the estimated manifold volume:

\begin{equation}
f(\boldsymbol{\phi}, \boldsymbol{\Phi})=\begin{cases}
1, \text{ if } \norm{\boldsymbol{\phi} - \boldsymbol{\phi}^\prime}_2 \leq \norm{\boldsymbol{\phi}^\prime - \text{NN}_k\left(\boldsymbol{\phi}^\prime, \boldsymbol{\Phi}\right)}_2 \text{ for any } \boldsymbol{\phi}^\prime \in \boldsymbol{\Phi}\\
0, \text{ otherwise.}
\end{cases}
\label{eq:manifold_estimate}
\end{equation}

Here, $\text{NN}_k\left(\boldsymbol{\phi}^\prime, \boldsymbol{\Phi}\right)$ returns the $k$th nearest feature vector to $\boldsymbol{\phi}^\prime$ in the set $\boldsymbol{\Phi}$.
\end{comment}
The improved precision is then defined as:

\begin{align}
\text{precision}(\boldsymbol{\Phi}_r, \boldsymbol{\Phi}_g) = \frac{1}{\abs{\boldsymbol{\Phi}_g}}\sum_{\boldsymbol{\phi}_g \in \boldsymbol{\Phi}_g}^{}f(\boldsymbol{\phi}_g, \boldsymbol{\Phi}_r),
\end{align}
where $f(\boldsymbol{\phi}, \boldsymbol{\Phi})$ is a binary function that identifies whether a sample $\boldsymbol{\phi}$ resides within the estimated manifold volume;

%These metrics determine whether a given image appears within the estimated manifold of the opposing set.
\end{metric}

\begin{metric}[Improved Recall]
\label{met:ir}
Correspondingly, the improved recall is defined as
\begin{align}
\text{recall}(\boldsymbol{\Phi}_r, \boldsymbol{\Phi}_g) = \frac{1}{\abs{\boldsymbol{\Phi}_r}}\sum_{\boldsymbol{\phi}_r \in \boldsymbol{\Phi}_r}^{}f(\boldsymbol{\phi}_r, \boldsymbol{\Phi}_g). \label{eq:knn_precision_recall}
\end{align}
\end{metric}

\begin{metric}[Inception Score]
\label{met:is}
The 'Inception Score' \citep{NIPS2016_8a3363ab} (IS) for $p_{gen}$ in relation to $p_{dis}$ is defined as:
\begin{align*}
IS(p_{gen}, p_{dis}) := \exp\left( \mathbb E_{x\sim p_{gen}}\left[
	  D_{KL} \left(p_{dis}(\cdot | x) \| \int p_{dis}(\cdot | x) p_{gen}(x)dx \right)
	  \right]\right).
\end{align*}
$p_{gen}$ is denoted as a probability distribution over $\Omega_X$ that is under evaluation. The discriminator is defined as a function $p_{dis}:\Omega_X \to M(\Omega_Y)$, where $M(\Omega_Y)$ encompasses all probability distributions on $\Omega_Y$. For any given image $x$ and label $y$, $p_{dis}(y|x)$ signifies the probability, assigned by the discriminator, of image $x$ possessing label $y$.
\begin{comment}
This can be equivalently expressed as:
\begin{align*}
\ln IS(p_{gen}, p_{dis}) := \mathbb E_{x\sim p_{gen}}\left[
		  D_{KL} \left(p_{dis}(\cdot | x) \| \mathbb E_{x\sim p_{gen}}[p_{dis}(\cdot | x)]\right)
		  \right]
\end{align*}

or

\begin{align*}
\ln IS(p_{gen}, p_{dis}) :=
		  H[\mathbb E_{x\sim p_{gen}}[p_{dis}(\cdot | x)]]
		  -\mathbb E_{x\sim p_{gen}}[ H[p_{dis}(\cdot | x)]]
\end{align*}

Here, $\ln IS$ is always nonnegative, in accordance with Jensen's inequality.
\end{comment}
\end{metric}

\begin{metric}[Frechet-Inception Distance (FID)]
\label{met:fid}
The "Fr\'{e}chet Inception Distance" (FID) $d(.,.)$ between the Gaussian with mean $(\Bm,\BC)$ derived from $p(.)$ and the Gaussian with mean $(\Bm_w,\BC_w)$ is defined as \citep{NIPS2017_8a1d6947}:

\begin{align}
d^2((\Bm,\BC),(\Bm_w,\BC_w))=\|\Bm-\Bm_w\|_2^2+  \TR \bigl(\BC+\BC_w-2\bigl(
\BC\BC_w\bigr)^{1/2}\bigr) \ .
\end{align}
It has been found that the FID is consistent with increasing disturbances and aligns with human judgment.
\end{metric}

\begin{metric}[Authenticity (AuthPct)]
\label{met:ap}
The {\it authenticity}~score~$A \in [0, 1]$ from \cite{alaa2022faithful} to quantify the rate by which a model generates {\it new} is defined as a mixture of densities as follows: 
\begin{align}
\mathbb{P}_g = A \cdot \mathbb{P}^\prime_g + (1-A) \cdot \delta_{g,\epsilon}, 
\label{authensc}
\end{align}
$\mathbb{P}^\prime_g$ symbolizes the generative distribution, excluding duplicated synthetic samples. $\delta_{g,\epsilon}$, a noisy distribution over training data, is expressed as $\delta_{g,\epsilon} = \delta_{g} \ast \mathcal{N}(0, \epsilon^2)$. $\delta_g$ is a discrete distribution for training data points in $\mathcal{D}_{real}$ and $\epsilon$ signifies a small noise variance. The model, as per Equation (\ref{authensc}), either draws a noisy training sample with probability $1-A$ or innovates a new sample with probability $A$.
\begin{comment}
$\mathbb{P}^\prime_g$ denotes the generative distribution, factoring in only non-duplicated synthetic samples. $\delta_{g,\epsilon}$ is defined as a noisy distribution over training data, given by $\delta_{g,\epsilon} = \delta_{g} \ast \mathcal{N}(0, \epsilon^2)$, where $\delta_g$ is a discrete distribution assigning an undefined probability mass to each point in $\mathcal{D}_{real}$. $\epsilon$ represents a small noise variance, and $\ast$ is the convolution operator. Essentially, Equation (\ref{authensc}) suggests that the model either samples from training data with probability $1-A$, incorporating noise, or generates a novel sample with probability $A$.
\end{comment}
\end{metric}

\begin{metric}[CTScore]
\label{met:ct}
The CTScore for data copying is defined by \cite{DBLP:journals/corr/abs-2004-05675} as:
\begin{align*}
    C_T(P_n, Q_m) \coloneqq  \frac{\sum_{\pi \in \Pi_\tau} P_n(\pi) Z_U\big(L_\pi(P_n), L_\pi(Q_m); T\big)}{ \sum_{\pi \in \Pi_\tau} P_n(\pi) }.
\end{align*}
The $z$-scored Mann-Whitney $U$ statistic, $Z_U$, is calculated for each cell $\pi$. The fractions of points in $\pi$ from $P_n$ and $Q_m$ are represented as $P_n(\pi)$ and $Q_m(\pi)$ respectively. $Z_U\big(L_\pi(P_n), L_\pi(Q_m); T\big)$ denotes the $Z_U$ test where $L_\pi(P_n)$ and $L_\pi(Q_m)$ are distances for points within $\pi$. Data-copying is measured for cells where representation by $Q$ exceeds the threshold $\tau$. $\Pi_{\tau}$ represents all cells in $\Pi$ where $Q_m(\pi) \geq \tau$. The summary statistic for data copying is an average across these cells.
\end{metric}

==> sections/5.Assessment/memo-old.tex <==
\begin{comment}
Similarly, 

Results

figure

Qualitative results

Implications: our model, other models, evaluation, relation to other



are well ...

an obligation for the generation of data in general and for medical data in particular, because of its sensitive content. 

While

We nonetheless evaluate degree of correspondence ...

Explain metrics
ahmed

ct score

inteprete results

include knn samples

For the quantitative evaluation of the ability to memorize training samples, we compute the measure of Authenticity (AuthPct) proposed in \citep{alaa2022faithful} and the measure to test data-copying (CTScore) from \citep{Meehan2020datacopy}. To evaluate visually the similarity of the training data, to generated samples, we perform a nearest neighbor search in the inception-v3 feature space of the training data. The resulting nearest neighbors are shown in \Cref{fig:image_generation}.
The results of the nearest neighbor search emphasizes the need for official regulatory guidelines on the appropriate use of synthetic data.
\end{comment}

\begin{comment}
\todo{Sampling with labelled and unlabelled data prevents the complete memorization of patients' data.}
%\section{Experiments on Privacy Validation}

\subsubsection{Training Data Memorization in Diffusion Models}
From a medical/anatomical perspective, data protection, and learning theory point of view, training data memorization in diffusion models for histopathological data is a critical concern. Diffusion Models (DMs) represent a class of parameterized Markov chains that effectively optimize the lower variational bound associated with the likelihood function \cite{sohl2015}. They can approximate complex distributions much more faithfully than GANs, and by extension, generate much more diverse samples, without sacrificing fidelity \cite{nichol2021}.

\subsubsection{Realism of Existing Privacy/Memorization Evaluation Protocols}
Existing privacy/memorization evaluation protocols for generative models are often questioned for their realism, especially in relation to access to train data. The protocols include measuring the consistency between real and fake data embedded with downstream models \cite{alaa2022}, comparison with inpainted areas \cite{carlini2023}, or forgotten examples detection \cite{jagielski2022}.

\subsubsection{Experiment Setup}
The experiment setup involves using appropriate metrics to evaluate quantitatively the degree of memorization. This includes an approach that compares k-nearest neighbors (knn) between training data and sampled data in a UMAP dimensionality reduced feature space of the generative model.




discussion

medical

data protection

ml

realism of eval protocol

access to train data
not access to raw data

metrics?

embedding - quant

embedding - qual
\end{comment}
